Sealer: In-SRAM AES for High-Performance and Low-Overhead Memory Encryption

To provide data and code confidentiality and reduce the risk of information leak from memory or memory bus, computing systems are enhanced with encryption and decryption engine. Despite massive efforts in designing hardware enhancements for data and code protection, existing solutions incur significant performance overhead as the encryption/decryption is on the critical path. In this paper, we present Sealer, a high-performance and low-overhead in-SRAM memory encryption engine by exploiting the massive parallelism and bitline computational capability of SRAM subarrays. Sealer encrypts data before sending it off-chip and decrypts it upon receiving the memory blocks, thus, providing data confidentiality. Our proposed solution requires only minimal modifications to the existing SRAM peripheral circuitry. Sealer can achieve up to two orders of magnitude throughput-per-area improvement while consuming 3x less energy compared to the prior solutions.

==> islped22-1/Background/background.tex <==
\vspace{-0.3cm}
\section{Background and Threat Model}
\vspace{-0.1cm}
% \esnote{I'd recommend using different folders for each section of the paper so it is easier to work and edit. Also clean out the template text to avoid confusion.}
%\vspce{-0.1cm}
\subsection{Advanced Encryption Standard}
\vspace{-0.1cm}
The Advanced Encryption Standard (AES) in cryptography, also known as Rijndael cryptography, is a block encryption standard.
The AES encryption process operates on a 4×4 matrix of bytes
%, also known as the ``state", 
whose initial value is a plaintext block (the element size in the matrix is one byte). 
Each AES encryption round (except the last one) consists of four steps where the output of each stage is used as an input for the next stage and described as follows.  
(1) \emph{AddRoundKey}: each byte in the matrix is XORed with the round key. Each round key is generated by the key generation scheme from a given cipher key. 
(2) \emph{SubBytes}: each byte is substituted with its corresponding byte in the S-box block using a nonlinear substitution function commonly implemented with lookup tables (LUTs). 
(3) \emph{ShiftRows}: a round-robin shift is performed for each row in the matrix. The first row is unchanged while each element of the second row are shifted to the left by 1 byte. Then for the third and fourth row, elements are shifted to the left by 2 and 3 bytes, respectively (see matrix D1 to D2 transformation in Figure \ref{AES_flow}). 
(4) \emph{Mixcolumns}: this step uses a linear transformation to fully mix the four bytes of each column. In AES, the \emph{MixColumns} stage is omitted from the last encryption loop and replaced with another \emph{AddRoundKey}.

The overall process of AES for a 128-bit plaintext is shown in Figure \ref{AES_flow}. First, the plaintext is XORed with the original cipher key for initialization. Then after 9 main rounds, each of which consists of \emph{AddRoundKey}, \emph{SubBytes}, \emph{ShiftRows}, and \emph{MixColumns}, and the final round without \emph{MixColumns}, the 128-bit ciphertext is generated.

\begin{figure}[htp]
\vspace{-0.3cm}
\centerline{\includegraphics[width=2.5in]{Background/aesflow-v2.pdf}}
\vspace{-0.3cm}
\caption{The steps of AES for a 128-bit plaintext.
% \esnote{some space, take the last three boxes and show then horizontally from left to right. Also make the transition lines bolder.}
}
\label{AES_flow}
\vspace{-0.5cm}
\end{figure}

\vspace{-0.3cm}
\subsection{Computing in SRAM}
\vspace{-0.1cm}
In-SRAM computing relies on the underlying bitline computation by activating more than one row in the SRAM subarray \cite{jeloka28NmConfigurable2016a,sadredini2020impala}. 
%Figure \ref{bitline} represents some of the logical operations that SRAM can support. 
The bitwise AND and NOR operations in SRAM are implemented directly by utilizing sense amplifiers (SAs) with multiple wordlines activated, as shown in Figure \ref{bitline}(a). 
The SA on the bitline ($BL$) can sense a voltage higher than $V_{ref}$ only if all the cells in the activated rows connected to the corresponding $BL$ contain `1'. 
This means the SA will sense `1', thus, achieving element-wise AND operation.
The SA on the bitline-bar ($\overline{BL}$) will sense a voltage higher than $V_{ref}$ only if all the cells in the activated rows connected to the corresponding $\overline{BL}$ contain `1', which, in turn, implies that all the cells in the activated rows connected to the corresponding $BL$ contain '0'.  
This means the SA will sense `1', thus, achieving element-wise NOR operation.
Using the logical bitwise AND and NOR operations, the XOR operation can be performed, as shown in Figure \ref{bitline}(b).
%by connecting the output of AND and NOR operations to the input of a NOR gate, as shown in Figure \ref{bitline}(b).

%'0' only if all the cells in the activated rows contain 0', that is, if all the cells passed by the bitline bar contain `1', the SA on the bitline bar side can sense a voltage higher $V_{ref}$, thus outputting 1 and implementing the element-wise NOR operation.

%What's more, based on the above two logical operations, the result of XOR operation can be successfully output by connecting the output of AND and NOR operations to the input of a NOR gate, as shown in Figure \ref{bitline}(b).


Many studies based on computing in SRAM have been proposed \cite{agaComputeCaches2017,eckertNeuralCacheBitserial2018,fujikiDualityCacheData2019,subramaniyanCacheAutomaton2017}.
% eckertNeuralCacheBitSerial2018,fujikiDualityCacheData2019,subramaniyanCacheAutomaton2017}.
%eckertNeuralCacheBitSerial2018
%jeloka28NmConfigurable2016
%zhaHyperApEnhancingAssociative2020
%khoramAlternativeAnalyticalApproach2018
%kangMultiFunctionalInMemoryInference2018
Cache Automaton uses a sense-amplifier cycling technique to read out multiple bits in one time slot, thus significantly reducing input symbol match time \cite{subramaniyanCacheAutomaton2017}.
Based on the described NOR, AND, and XOR operations, Compute Cache extends the logical operations by slightly modifying the SA design in \cite{agaComputeCaches2017}.
%Neural Cache \cite{eckertNeuralCacheBitSerial2018} implements addition, multiplication, and reduction by reconstructing the SRAM structure based on Compute Cache.
In this paper, we utilize the XOR functionality presented in \cite{agaComputeCaches2017}, and slightly modify it (similar to \cite{gencache}) to be able to perform the shift operation (required for the proposed fused \emph{ShiftRows} and \emph{MixColumns} stages) in place without the need to store the intermediate result back into the subarray, thus, reducing processing cycles.  

\begin{figure}[htp]
\vspace{-0.3cm}
\centerline{\includegraphics[width=1.7in]{Background/bitline.pdf}}
\vspace{-0.3cm}
\caption{The XOR bitline operation using 6T SRAM cells.}
\label{bitline}
\vspace{-0.5cm}
\end{figure} 

\begin{comment}
SRAM has lower access latency compared to DRAM and is typically used as on-chip cache for CPU. 
A number of in-memory computing researches have been proposed on cache \cite{agaComputeCaches2017,jeloka28NmConfigurable2016,eckertNeuralCacheBitSerial2018,khoramAlternativeAnalyticalApproach2018,zhaHyperApEnhancingAssociative2020,fujikiDualityCacheData2019,kangMultiFunctionalInMemoryInference2018}. 
The basic logical operations in the cache are element-wise AND and NOR, which can be implemented directly by utilizing SA with multiple wordlines activated \cite{jeloka28NmConfigurable2016}. 
Based on these two operations, Compute Cache extends the logical operations to $copy$, $xor$, etc. by slightly modifying SA \cite{agaComputeCaches2017}.
Neural cache \cite{eckertNeuralCacheBitSerial2018} implements addition, multiplication, reduction, etc. by reconstructing the cache structure based on Compute Cache.
\end{comment}

\vspace{-0.2cm}
\subsection{Threat Model}\label{sec:threatmodel}
\vspace{-0.1cm}
Similar to the state-of-the-art secure memory architectures~\cite{gueronMemoryEncryptionEngine2016b}, we assume the only trusted component is the processor chip and we do not expand the TCB of the system. Therefore, bus and memory are vulnerable and untrusted. We assume the attacker has physical access to the system and can snoop on the bus, or scan the memory.
%to read the data. 
This work proposes high-performance encryption for protecting data confidentiality. Addressing timing channels, replay attacks, and access pattern leakage threat models are left for future work.

%%\vspce{-0.2cm}

==> islped22-1/Conclusion/conclusion.tex <==
\vspace{-0.3cm}
\section{Conclusion}
\vspace{-0.1cm}
%\esnote{Most likely we need to make the references more compact to free up some space. A few suggestions: page numbers (i.e., pp. can be removed), Conference acronym name can be used instead of entire conference name, and authors name can be changed to the "et al." format. For some other conferences (such as MICRO or HPCA), references are counted towards page limitation, so we do not need to make the references compact for those conferences.}

In this paper, we propose \emph{Sealer}, a real-time low-overhead in-SRAM AES engine to encrypt the plaintext on a CPU chip with narrowed trusted computing base. By efficiently mapping the algorithm to the \emph{Sealer} architecture at a finer granularity, data movement is significantly reduced.
Our evaluation results show significant performance (up to 323$\times$) and throughput-per-area (up to 91$\times$) improvement over the state-of-the-art in-memory and specialized encryption engines. Future work will extend \emph{Sealer} to provide data integrity as well as access pattern protection.
%With 18$\times$ architectural contribution and 18$\times$ technology benefits to performance, Sealer can achieve up to 323$\times$ latency reduction and up to 91$\times$ throughput-per-area improvement over prior solutions.

% high-performance and energy-efficient in-cache memory encryption engine, Sealer. 
% By taking advantage of the high parallelism of the SRAM subarray and the bitline computational capability, Sealer can achieve real-time data encryption on the chip with minimal modifications to the peripheral circuity. 
% Compared with other AES engines based on the emerging NVM technology, Sealer can speed up the encryption of one data block by up to 1700x and obtain 5x throughput over a unit area.
% For future work, we will extend Sealer to provide data integrity and access pattern protection in addition to data confidentiality.

% \begin{itemize}
%     \item We present \textit{Sealer}, a real-time in-SRAM AES engine to provide data confidentiality by encrypting the plaintext on the CPU chip and narrowing the TCB. Our proposed architecture effectively stores the required data and matrices for encryption into the same SRAM subarray. This allows the peripherals and resources to be shared for different computation and communication requirements, thus, reducing performance and hardware overhead. 
%     %and prevent physical attacks, such as bus snooping and cold boot attacks. Our design requires minimal change to the SRAM array structure.   
%     %\item ... by narrowing the trusted computing base (TCB) to the inside of the CPU package ... to ensure confidentiality ... encrypts the plaintext using AES algorithm and sends the encrypted data to DRAM.
%     \item We present an algorithm and architecture methodology to efficiently map the AES algorithm to the Sealer architecture. By fusing the \textit{SubBytes} and \textit{ShiftRows} stages in AES, we can interleave the computation at a finer granularity and maximally exploit on-the-fly computation to significantly reduce data movement and the number of write cycles into the subarrays.  
%     \item We compare \textit{Sealer} with several on-chip and in-memory AES encryption engines and show that our solution has up to \textcolor{red}{323$\times$} performance benefit and up to \textcolor{red}{91$\times$} throughput-per-area improvement over prior solutions. Furthermore, to separate the architectural and technology contribution of \textit{Sealer}, we evaluate, AIM, an NVM-based AES engine, on SRAM subarrays (AIM-SRAM) and find that our solution achieves 18$\times$ higher performance than AIM-SRAM due to architectural contribution and 18$\times$ better performance due to technology benefits.
    
% \end{itemize}

%\section*{Acknowledgment}
%\vspace{-0.0cm}

==> islped22-1/Evaluation/eval.tex <==
\vspace{-0.2cm}
\section{Evaluation}\label{sec:evaluation}
\vspace{-0.1cm}

\subsection{Evaluation Methodology}
% \vspace{-0.1cm}
% \esnote{a table for L3 cache energy (read, write, xor) - Use Table V in compute cache.}\\

% \esnote{Which technology node}\\

% \esnote{Check if we can compare with InvisiMem}\\
% \jynote{InvisiMem offers no exact parameters about latency and energy. Only the overhead (\%). I think we cannot compare with InvisiMem.} 
% \esnote{I also checked and I agree. If we find a suitable place, we can briefly mention why we are not comparing with InvisiMem}
% \jynote{I added a sentence in this subsection. 
% "We do not compare here with InvisiMem \cite{agaInvisiMemSmartMemory2017} because the structure of the smart memory with logic layers used by InvisiMem is very different from cache, NVM, and DRAM."}

In this section, we evaluate the performance, throughput-per-area and energy/power of \emph{Sealer} 
%assuming 256x256 subarrays 
and compare it to prior in-memory encryption solutions \cite{xieSecuringEmergingNonvolatile2018,wangDWAESDomainwallNanowirebased2016} and on-chip memory encryption implementations \cite{hamalainenDesignImplementationLowarea2006,mathew53GbpsNativeGF2010}.
%\jynote{For Question 2: Compared to unmodified SRAM, the hardware overhead of Sealer is less than 1.55\%. And since the unmodified SRAM cannot perform computation in subarray, we compare \textit{Sealer} here with other ASIC designs and in-memory designs.}
AIM architecture\cite{xieSecuringEmergingNonvolatile2018} is implemented in-MRAM (\emph{AIM-NVM}) and \emph{Sealer} utilizes
%64Kb
SRAM-based subarrays. To decouple architectural contribution from the technology contribution and have an apples-to-apples comparison between AIM and \emph{Sealer}, we model and evaluate the architecture of AIM in SRAM (\textit{AIM-SRAM}).
The area overhead evaluation presented in the AIM is based on relative numbers. To directly compare the area overhead of AIM-NVM and AIM-SRAM with \emph{Sealer}, we use NVSim \cite{dongNVSimCircuitlevelPerformance2012} to obtain the absolute area parameters for the peripherals used in AIM-NVM. 
The read/write access latency to a $256\times256$ 6T SRAM subarray is 163 $ps$, and 
an XOR operation in SRAM costs 489 $ps$, which are extracted from the SPICE simulations with 28nm SOI CMOS process \cite{subramaniyanCacheAutomaton2017,agaComputeCaches2017}. 
DESTINY \cite{destiny} is used to evaluate the energy and power consumption of SRAM-based and NVM-based designs.
%\jynote{For Question 15: Full system simulation including the synthesis of placement and routing is our next step.}
%\jynote{For Question 3: For off-chip encryption/decryption designs such as AIM\cite{xieSecuringEmergingNonvolatile2018} and DW-AES\cite{wangDWAESDomainwallNanowirebased2016}, we consider them to be insecure. According to our threat model in Section \ref{sec:threatmodel}, the plaintext will never appear on the memory bus, thus we o not consider the data movement overhead from off-chip DRAM to on-chip SRAM.}
%Optimistic parameters of NVM is from \cite{patrigeonDesignEvaluation28nm2019} and the implementation of LUT is based on \cite{jeloka28NmConfigurable2016a}.

\begin{figure}[tp]
\vspace{-0.3cm}
\centerline{\includegraphics[width=3.3in]{Implementation/mixcolumns-v3.pdf}}
\vspace{-0.3cm}
\caption{Example of \emph{MixColumns} stage.
%: substep (a) calculates $T_0$, substep (b) calculates $B_{0,0}$.
}
% \jynote{Need polish, the alignment of blocks, shrink block size, might add some peripheral circuit}
\label{mixcolumn}
\vspace{-0.6cm}
\end{figure} 
% Table \ref{l3-table} shows the energy and latency of one read and write access to a $256\times256$ SRAM subarray, as well as the energy and latency of performing parallel XOR operation in one subarray, following \cite{subramaniyanCacheAutomaton2017,agaComputeCaches2017}.
% These numbers are extracted from the SPICE simulations with 28nm SOI CMOS process assuming $6T$ SRAM cell structure. 

% \vspace{-0.2cm}
% \begin{table}[htp]
% 	\caption{L3 cache energy and latency per access}
% 	\centering
% 	\vspace{-0.2cm}
%   \begin{adjustbox}{width=1.4in}
%     \begin{tabular}{|c|c|c|c|}
% 		\hline
% 		 metrics  & write & read & XOR \\
% 		\hline
% 		Energy (pJ) & 2852 & 2452 & 1672 \\
% 		\hline
% 		Latency (ps) & 163 & 163 & 489 \\
% 		\hline
% 	\end{tabular}
% 	\label{l3-table}
%   \end{adjustbox}
% \vspace{-0.3cm}
% \end{table}


%Here we do not compare with InvisiMem \cite{agaInvisiMemSmartMemory2017} because the architecture and memory type are both different of the smart memory with logic layers used by InvisiMem is very different from SRAM, NVM, and DRAM.
%We do not compare here with InvisiMem \cite{agaInvisiMemSmartMemory2017} because InvisiMem does not accelerate the AES algorithm but uses a synthesis tool to synthesize the AES engine. However, his research on address encryption is informative. We will research this area in the future.

The baselines are (1) EE-1 \cite{hamalainenDesignImplementationLowarea2006}, which introduces an AES encryption based on a dedicated engine for low power consumption at 290 MHz, (2) EE-2 \cite{mathew53GbpsNativeGF2010}, which presents a high-frequency integrated circuit encryption engine at up to 2.13 GHz, (3) DW-AES \cite{wangDWAESDomainwallNanowirebased2016}, which uses domain-wall nanowires to implement AES encryption in NVM at 30MHz, (4) AIM-NVM, and (5) AIM-SRAM.% which is our implementation of AIM-NVM architecture on 6T SRAM subarrays.

% The baselines for comparison against \emph{Sealer} are: 
% \begin{enumerate}
%     \item EE-1 \cite{hamalainenDesignImplementationLowarea2006} introduces an AES encryption based on dedicated hardware engine for low power consumption at 290 MHz.
%     \item EE-2 \cite{mathew53GbpsNativeGF2010} presents a high-frequency integrated circuit encryption engine which can perform up to 2.13 GHz.
%     %\hnnote{I just noticed these EE1 and EE2 are very old papers! Older than SGX! I can not even justify it in related work. Reviewers will ask about why we are evaluating our design against these papers... }
%     \item DW-AES \cite{wangDWAESDomainwallNanowirebased2016} uses domain-wall nanowires to implement AES encryption in NVM at 30MHz.
%     \item AIM-NVM \cite{xieSecuringEmergingNonvolatile2018} is an implementation of AES encryption in NVM with subarray-level parallelism at 30 MHz. %\jynote{calculated by the read latency 31.97ns in AIM paper.}
%     \item AIM-SRAM is our implementation of AIM-NVM architecture on 6T SRAM subarrays.

% \end{enumerate}

\vspace{-0.2cm}
\subsection{Latency Analysis} \label{PerformanceAnalysis}
\vspace{-0.1cm}
Figure \ref{combine} compares the data encryption latency of different solutions normalized to the \emph{Sealer} latency for 24 data blocks (384 bytes) and for 192 data blocks (3072 bytes, which is approximately the size of one cache slice in L3 \cite{lempel2ndGenerationIntel2011}). 
\emph{Sealer} has 30$\times$ (243$\times$), 1.22$\times$ (9.8$\times$), and 1880$\times$ (15040$\times$) lower latency than EE-1, EE-2, and DW-AES, respectively, for encrypting 24 data blocks (192 data blocks).
%Sealer is just slightly less than that of EE-2 in one subarray, 
For all these solutions, \emph{Sealer's} performance improves significantly when increasing the memory capacity because of the intrinsic bit-level and subarray-level parallelism in memory. 
For example, EE-2 can operate on only four blocks in parallel, 
%every five clock cycles
while \emph{Sealer} can encrypt 192 data blocks simultaneously when utilizing the 2MB SRAM. %\jynote{192 = (2MB/64KB) x 6.}
In general, in-memory solutions (\emph{Sealer}, AIM-NVM, and AIM-SRAM) provide higher parallelism than dedicated hardware engines.  
%As shown in Figure \ref{combine}, generally in-memory implementations can handle bulk encryption better than dedicated hardware cores due to the high parallelism of in-memory computing. 

\begin{comment}
Figure \ref{combine} compares the data encryption latency of different solutions normalized to the \emph{Sealer} latency for 6 data blocks (96 bytes) and for 192 data blocks (3072 bytes, which is approximately the size of one cache slice in L3 \cite{lempel2ndGenerationIntel2011} in \emph{Sealer}). 
\emph{Sealer} has 19$\times$ (608$\times$), 1.02$\times$ (24$\times$), and 1174$\times$ (37572$\times$) lower latency than EE-1, EE-2, and DW-AES for encrypting 6 data blocks (192 data blocks).
%\emph{Sealer} is just slightly less than that of EE-2 in one subarray, 
For all these solutions, \emph{Sealer} performance improves significantly when increasing the memory capacity because of the intrinsic bit-level and subarray-level parallelism in memory. 
For example, EE-2 can operate on only four blocks in parallel, 
%every five clock cycles
while \emph{Sealer} can encrypt 192 data blocks simultaneously when utilizing the 2MB SRAM. %\jynote{192 = (2MB/64KB) x 6.}
In general, in-memory solutions (\emph{Sealer}, AIM-NVM, and AIM-SRAM) provide significantly higher parallelism than dedicated hardware engines (EE-1, and EE-2).  
%As shown in Figure \ref{combine}, generally in-memory implementations can handle bulk encryption better than dedicated hardware cores due to the high parallelism of in-memory computing. 
\end{comment}


\begin{figure}[htp]
\vspace{-0.3cm}
\centerline{
\includegraphics[width=3.1in]{Evaluation/combine.pdf}
}
\vspace{-0.3cm}
\caption{Latency comparison among different baselines normalized to \emph{Sealer} for encrypting 24 and 192 data blocks.}
\label{combine}
\vspace{-0.4cm}
\end{figure}

\emph{Sealer} has almost 6.5$\times$ lower latency than AIM-SRAM (architectural contribution of \emph{Sealer} compared to AIM). 
This is because the required number of cycles for encrypting six data blocks in a subarray in AIM-SRAM is almost 6.5$\times$ higher than \emph{Sealer}, as shown in Figure \ref{cyclenumber}. 
Figure \ref{cyclenumber} compares the cycle breakdown for different stages in \emph{Sealer} and AIM. \emph{AddRoundKey} stage has the same number of cycles in both architectures. However, the fused \emph{SubBytes} and \emph{ShiftRows} stage in \emph{Sealer} requires 59.5\% fewer cycles than the total cycles for \emph{SubBytes} and \emph{ShiftRows} stages in AIM. This benefit is enabled by storing all required data (i.e., data blocks, S-box, round keys, and intermediate data) in the same subarray, which facilitates computation fusion among different stages, thus, resulting in fewer write cycles. 
Moreover, in the \emph{MixColumns} stage, unlike AIM which uses additional LUTs, \emph{Sealer} utilizes the existing rows and peripherals in the under-processed subarray to store intermediate results, thus, avoiding the bandwidth bottleneck of moving data between subarrays and limited LUTs.
%AIM architecture uses additional LUTs to store the S-box and intermediate data, and a single LUT allows only one-byte access at a time unless replicated. 
Increasing the number of LUTs can provide more parallelism in AIM, however, it significantly increases area overhead, thus, decreasing throughput-per-area. 

\emph{Sealer} has 107$\times$ and 323$\times$ lower latency than AIM-NVM for encrypting 24 and 192 data blocks, respectively.
The latency reduction for encrypting 24 data blocks comes from the architectural contribution (about 6$\times$ due to the data layout and stage fusion) and technology contribution (about 18$\times$ due to the choice of SRAM compared to NVM) in \emph{Sealer}. 
% \emph{Sealer} has almost 107$\times$ lower latency than AIM-NVM for encrypting 24 data blocks, which comes from the architectural contribution (about 6$\times$) and technology contribution (about 18$\times$ due to the choice of SRAM compared to NVM) in \emph{Sealer}. 
%\jynote{I corrected the latency figure. Now \emph{Sealer} has 107$\times$ (323$\times$), lower latency than AIM-NVM for encrypting 24 data blocks (192 data blocks). The reason why I use 24 data blocks to show our advantage is that the performance of EE-2 is better than \emph{Sealer} for encrypting 6 data blocks.}
%Moreover, The increasing latency reduction for 192 data blocks is from the architectural contribution which support parallel encryption in large amount. 
Overall, \emph{Sealer} presents a low latency encryption solution, which is suitable for real-time encryption.  

% As for encrypting 192 data blocks, \emph{Sealer} has 323$\times$ lower latency than AIM-NVM. The increasing latency reduction is from the increasing architectural contribution. \emph{Sealer} can encrypt 192 data blocks parallelly while AIM-NVM can only handle 64 data blocks at the same time.
% Overall, \emph{Sealer} presents a low latency encryption solution, which makes it suitable for real-time encryption.  

\begin{comment}
The \emph{Sealer} has almost 270$\times$ lower latency than AIM-NVM, which comes from the architectural contribution (about 3$\times$) and technology contribution (about 90$\times$ due to the choice of SRAM compared to NVM) in \emph{Sealer}. \jynote{I corrected the latency of DW-AES and AIM-NVM for encrypting 192 data blocks shown in Fig. 6. Now \emph{Sealer} has 107$\times$ (323$\times$), lower latency than AIM-NVM for encrypting 6 data blocks (192 data blocks). The DW-AES-related part has been modified.}
Overall, \emph{Sealer} presents a low latency encryption solution, which is suitable for real-time encryption.  
\end{comment}

\begin{figure}[htp]
\vspace{-0.3cm}
\centerline{
\includegraphics[width=2.2in]{Evaluation/cycletime.pdf}
}
\vspace{-0.3cm}
\caption{Breakdown of processing cycles in AIM-SRAM and \emph{Sealer} for encrypting 6 data blocks.}
\label{cyclenumber}
\vspace{-0.3cm}
\end{figure}

% \begin{figure}[htp]%
%     \centering
%     \subfloat[Breakdown of processing cycles in AIM-SRAM and \emph{Sealer} for encrypting 6 data blocks.]{{\includegraphics[width=3.2in]{Evaluation/cyclenumber-v4.pdf} }}%
    
%     \subfloat[Throughput comparison among AIM-NVM, AIM-SRAM, and \emph{Sealer} for encrypting 192 data blocks.]{{\includegraphics[width=3.2in]{Evaluation/throughput.pdf} }}%
%     \caption{Energy \& power comparison among \emph{Sealer}, AIM-NVM, and AIM-SRAM for encrypting 24 and 192 data blocks.}%
%     \label{energy}%
% \end{figure}

%In the final MixColumns stage, the \emph{Sealer} does not use LUTs to store intermediate variables and so will not encounter the bandwidth bottleneck problem encountered by AIM. 

%Next, the AIM will first execute the LUT-based SubBytes stage.
%After the LUT substitution is executed, the LUT can output the result to the correct location by controlling the DEMUX to pass the ShiftRows stage.

%Among in-memory implementations, the latency of DW-AES increases from 195x to 587x with the increasing size of encryption data due to the limited parallelism of DW-AES.

%It can be seen that for a data block, the number of clocks used by the \emph{Sealer} is about one-third of that of the AIM.


%\emph{Sealer} outperforms DW-AES, NVM-based and cache-based implementations of AIM in both scenarios of subarray and cache slice. 
%\emph{Sealer} achieves a speedup of up to 195x and 270x compared to the DW-AES and NVM-based AIM, respectively, in one subarray. 
%This is because NVM, despite high parallelism, cannot effectively accelerate the encryption in a single subarray, which is why NVM-based encryption engines 


% \esnote{a graph to compare latency between \emph{Sealer}, AIM, ... - See Fig 12, AIM paper}
% \esnote{How many cycles, frequency, and delay for encrypting a data block}
% \jynote{If possible, count the cycle number of AIM. So we can decrease the capacity from 1 GB to 6 blocks. Write a mail to Mimi for a number of the clock cycle.}

% \begin{figure}[htp]
% \centerline{
% \includegraphics[width=3.4in]{Evaluation/latency.eps}
% }
% \caption{Comparison of latency between different baselines and our design. }
% \label{latency}
% \end{figure}

%\jynote{The latency of AIM-NVM for one data block is calculated by dividing 0.018 seconds by (32x12). 0.018 seconds is the time consumption mentioned in the AIM paper for encrypting 1 GB memory. Since the chip capacity of MRAM is 256 Mb, to encrypt 1 GB memory, AIM needs to run 32 times on this MRAM. Also, to encrypt one data block, there are 11 key matrices attached to this data block (if no key is shared). Thus, to encrypt 1 GB memory, AIM needs to run 32x12 times on one 256 MB MRAM chip. So by dividing 0.018 seconds by 32x12, the result will be the latency of AIM-NVM for one data block.}

% \begin{figure}[htp]
% \centerline{
% \includegraphics[width=3.4in]{Evaluation/latency.pdf}
% }
% \caption{Comparison of latency between different baselines normalized to \emph{Sealer} for one subarray.}
% \label{latency}
% \end{figure}

% \begin{figure}[htp]
% \centerline{
% \includegraphics[width=3.4in]{Evaluation/latency-slice.pdf}
% }
% \caption{Comparison of latency between different baselines normalized to \emph{Sealer} for an 2MB L3 cache slice.}
% \label{latency-slice}
% \end{figure}

% As shown in Figure \ref{latency}, the EE-1 and EE-2 consume 37.025 and 0.039383 seconds for encryption of 1-GB data, respectively.
% AIM baseline has different latency based on different memory technology. 
% Here we show the latency with phase-change memory (PCM) and magnetic random access memory (MRAM).
% The chip capacity of PCM is 1 Gb while MRAM has 256 Mb per chip.
% If the memory is implemented with PCM and MRAM, the encryption speed of AIM can reach 21 seconds and 1.2 seconds, respectively.
% When the bank-independent encryption is enabled, AIM-B can encrypt the entire memory in 2.66 seconds and 0.15 seconds with PCM and MRAM.
% When parallelism at the subarray level is allowed, AIM-S can encrypt the entire memory of PCM and MRAM in 0.33 seconds and 0.018 seconds, respectively.

% In addition to existing designs, we also have an implementation of AIM with cache computing.
% For encrypting 1-GB data, the AIM with cache computing costs 32.509 or 31.087 seconds when only one block can perform encryption or the whole subarray is available.
% Our design achieves the speed of 11.68 or 4.86 seconds if encryption can be mapped into one block or one subarray, respectively.

\vspace{-0.4cm}
\subsection{Throughput Normalized to Area} \label{throughput}
\vspace{-0.1cm}
Figure \ref{throughput-slice} compares the throughput-per-area for \emph{Sealer}, AIM-NVM, and AIM-SRAM.
\emph{Sealer} has 7.2$\times$ higher throughput per unit area than AIM-SRAM. 
These benefits come from the fact that (1) \emph{Sealer} only incurs negligible extra overhead to the SRAM arrays by sharing the memory resources and peripheral among different stages of computation and communication, while AIM-SRAM requires additional hardware components, such as LUTs and bundles of MUX/DEMUXes, and (2) \emph{Sealer} utilizes an efficient algorithm/ architecture methodology to fuse different computational stages, which maximizes on-the-fly computation and minimizes data movement.
\emph{Sealer} can also achieve more than 91$\times$ throughput per unit area compared to the AIM-NVM. 
Although the area consumption of AIM-NVM is lower than \emph{Sealer}, the frequency of \emph{Sealer} is 133$\times$ higher than AIM-NVM; thus, resulting in higher throughput. 
% {4Ghz vs 30MHz} 
%due to the high-density of MRAM, thus \emph{Sealer} has better throughput per unit area.
%Note that for a fair comparison, we shrink the capacity of AIM-NVM from 32MB \cite{xieSecuringEmergingNonvolatile2018} to 2MB, the same as \emph{Sealer} and AIM-SRAM.



%On the other hand, AIM implements the AES with bandwidth-limited LUTs, while \emph{Sealer} uses the inherent subarrays to store S-box and intermediate data without bandwidth limitation.
%The AIM-SRAM outperforms AIM-NVM by about 13$\times$ in terms of the throughput per unit area mostly because of the architectural contribution in removing LUTs and technology contribution in higher frequency.

\begin{figure}[htp]
\vspace{-0.3cm}
\centerline{
\includegraphics[width=2.7in]{Evaluation/throughput.pdf}
}
\vspace{-0.3cm}
\caption{Throughput comparison among AIM-NVM, AIM-SRAM, and \emph{Sealer} for encrypting 192 data blocks.}
%\esnote{I think if you make this horizontal, we can save some space}\jynote{Added. If we want more space, I can crop each figure to spare some space.}
\label{throughput-slice}
\vspace{-0.4cm}
\end{figure}

% Our design can reach the best throughput among all the designs mentioned above with the same memory capacity.
% Assume the unit capacity is 64 Kb.
% The basic AIM baseline achieves up to 0.10\% of the throughput of our design.
% The throughput of the AIM-S with the highest parallelism is only 6.60\% of our design.
% The AIM with cache computing shows the highest throughput among all the baselines which is 15.65\% of our design.

% \begin{figure}[htp]
% \centerline{\includegraphics[width=3.4in]{Evaluation/chart (7).pdf}}
% \caption{Throughput between different EE-2 and our design per unit area ($m^2$). }
% \end{figure}

% \begin{figure}[htp]
% \centerline{\includegraphics[width=3.4in]{Evaluation/chart (8).pdf}}
% \caption{Throughput between EE-1 and our design per gate. }
% \end{figure}
\vspace{-0.3cm}
\subsection{Energy/Power Analysis}
\vspace{-0.1cm}
\begin{comment}
Figure \ref{energy} compares the energy and power of Sealer, AIM-NVM and AIM-SRAM when encrypting 24 and 192 data blocks. In terms of energy consumption, benefiting from NVM's inherent low energy consumption for reading and writing, AIM-NVM consumes 10\% of \emph{Sealer}'s energy consumption to complete encryption. However, when we eliminate the technical advantages of the NVM-based design by transforming it into the SRAM-based design (AIM-SRAM), \emph{Sealer} achieves an 74.07\% reduction in energy consumption due to the architectural design advantages. 
\end{comment}

Figure \ref{energy} compares the energy and power of Sealer, AIM-NVM, and AIM-SRAM when encrypting 24 and 192 data blocks.
To complete the encryption, \textit{Sealer} consumes 3$\times$ less energy compared to AIM-NVM and AIM-SRAM, thanks to our fusion scheme and the reduction of LUT queries.
The energy consumption of AIM-SRAM is slightly lower than AIM-NVM. This is because the \emph{MixColumns} stage, which has the highest number of operations during encryption in the AIM architecture, contains a large number of write operations (the write dynamic energy of AIM-NVM is higher than the read dynamic energy).  
%Even though the read dynamic energy of AIM-NVM is lower, due to the relatively higher write dynamic energy and large quantity of write operations, the total energy is slightly higher than AIM-SRAM.
Sealer has 34$\times$ and 2$\times$ higher power consumption compared to AIM-NVM and AIM-SRAM, respectively. This is because \emph{Sealer} has a higher operational frequency and also maximizes computational parallelism so that almost all units are activated and computing, which greatly increases compute/memory unit utilization. However, the other two designs have all other computing and memory units idle when querying the lookup table.
%\jynote{For Question 14: By trading power, \textit{Sealer} achieves up to two orders of magnitude throughput-per-area improvement while consuming 3$\times$ less energy compared to prior solutions.}

\begin{figure}[htp]%
\vspace{-0.5cm}
    \centering
    \subfloat{{\includegraphics[width=4cm]{Evaluation/energy.pdf} }}%
    \subfloat{{\includegraphics[width=4cm]{Evaluation/power.pdf} }}%
    % \subfloat{{\includegraphics[width=4.5cm]{Evaluation/energy-max.pdf} }}%
    % \subfloat{{\includegraphics[width=4.5cm]{Evaluation/power-max.pdf} }}%
    % \subfloat{{\includegraphics[width=4.5cm]{Evaluation/energy-3d.pdf} }}%
    % \subfloat{{\includegraphics[width=4.5cm]{Evaluation/power-3d.pdf} }}%
    \vspace{-0.3cm}
    \caption{Energy \& power comparison among \emph{Sealer}, AIM-NVM, and AIM-SRAM for encrypting 24 and 192 data blocks.}%
    \label{energy}%
\vspace{-0.2cm}
\end{figure}

\begin{comment}
\subsection{Energy/Power Analysis}
Figure \ref{energy} compares energy consumption of \emph{Sealer} and AIM-NVM normalized for encrypting 6 data blocks. 
Compared to AIM-NVM, \emph{Sealer} consume about 4$\times$ lower energy. The energy benefits are \emph{Sealer} comes from the reduced data movement in \emph{Sealer} (i.e., data and computation is located in the same subarray). \esnote{Not sure if this energy comparison is reliable as access to NVM array consumes significantly less energy} \jynote{yes, you are right. The power of AIM-NVM is very low. However, since the latency of AIM-NVM is very high. So the energy for encrypting 6 data blocks in AIM-NVM is higher than ours. The assumption here is the power of AIM-NVM will not decrease with the decreasing number of encryption data. If the AIM-NVM is in a small capacity with lower power, our energy consumption will be higher than that of AIM-NVM.}

%Sealer costs less energy than AIM-NVM, only consuming a quarter of the energy consumed by AIM-NVM. 
%Although when bitline computing is enabled, the energy consumption for reading one bit in SRAM is much larger than that for reading a bit in the NVM (4.7 PJ v.s. 0.03 PJ), Sealer can beat AIM-NVM in terms of energy saving.
%The reason is that the data movement is reduced due to our use of step fusion of SubBytes and ShiftRows. 
%In addition, since only a subarray and peripheral circuitry, are used in the evaluation, and the structure of "mat", which consists of several subarrays, is not used to improve parallelism as in AIM \cite{xieSecuringEmergingNonvolatile2018}, Sealer reduces a large quantity of energy consumed by the interconnection between subarrays compared to the AIM.

\begin{figure}[htp]
\centerline{
\includegraphics[width=2.4in,height=0.9in]{Evaluation/energy.pdf}
}
\caption{Energy comparison between \emph{Sealer} and AIM-NVM normalized for encrypting 6 data blocks. \esnote{make this horizontal to save space}\jynote{added.}}
\label{energy}
\end{figure}
\end{comment}


==> islped22-1/Implementation/implementation.tex <==
\vspace{-0.4cm}
\section{Implementation}
\vspace{-0.1cm}
\subsection{Data Organization}
\vspace{-0.1cm}

%Therefore, in a $256\times256$ subarray, we can fit 6 \emph{Tiles} in the same set of rows and 51 \emph{Tiles} in the same set of columns. 
\begin{figure}[htp]
\vspace{-0.3cm}
\centerline{\includegraphics[width=3.2in]{Implementation/overall-v15.pdf}}
\vspace{-0.5cm}
\caption{(a) Data organization in one subarray. (b) The detailed structure of the first S-box and data (Tile 0) with three inputs of AES encryption algorithm: S-box (256-row, 8-bit), 128-bit plaintext and 128-bit cipher key. (c) The structure of the sense amplifier to support XOR and shift operations.}
% \caption{(a) The XOR of bitline computing in the AddRoundKey step. (b) The decoder translates the XORed result into row index and column index to activate the corresponding wordline and bitlines. The result will be sensed by SA and output to the location following the requirements of the ShiftRows step. (c) The results after the ShiftRows are multiplied by two using bit-shift.}
\label{overall}
\vspace{-0.9cm}
\end{figure}


In this paper, an efficient implementation of the AES algorithm is accomplished using bitline computing of SRAM arrays, and can be realized by re-purposing a portion of the L3 cache or by replacing the existing on-chip encryption hardware. 
%By using two decoders outside the subarray, different wordlines can be activated simultaneously. In this case, the SA logic is used to perform XOR operations on the bits of the same bitline. 
To efficiently utilize bitline computing, we organize the S-box, plaintext, keys, and intermediate data required by the AES algorithm in the same subarray, as shown in Figure \ref{overall}(a).
We assume $256\times256$ SRAM subarrays, following Intel’s SandyBridge L3 cache structure \cite{lempel2ndGenerationIntel2011}. 
As depicted in Figure \ref{overall}, each subarray consists of 6 \emph{Tiles}, where each \emph{Tile} can store 51 data blocks ($Row[0]-Row[203]$ - each data block requires four rows), one set of round keys ($Row[204]-Row[247]$), and intermediate data required for \textit{MixColumns} stage ($Row[248]-Row[253]$).
The first 8 columns of the \emph{Tile} are used to hold the S-box.  
All the data blocks arranged in the same set of rows can encrypt/decrypt data in parallel (i.e., 6 data blocks per subarray). Data blocks in the same \emph{Tile} cannot be computed parallelly due to the shared bitlines.
 
The S-box is originally a 16$\times$16 matrix where each element is an 8-bit data. 
To avoid adding the extra LUT logic in the SRAM structure for S-box substitution in the \emph{SubBytes} stage, and also to eliminate the communication and wiring overhead between the data block subarrays and the LUTs, \emph{Sealer} proposes to re-organize the S-box into a matrix of 256 rows where each row has an 8-bit element (as shown in Figure \ref{overall}(b) - the blue matrix) and utilize the same subarray as the plaintext and round keys are located. The memory decoder is used to decode the 8-bit input data to select the corresponding element for the substitution. This brings two advantages in \emph{Sealer} compared to the prior work, AIM \cite{xieSecuringEmergingNonvolatile2018}, from the architectural aspect; (1) all the required data for performing the encryption is within the same subarray, and this brings the opportunity to fuse computation in different stages while the data is read into SA, and also perform intermediate data generation on-the-fly without the need to write them back into the subarray, thus, reducing the total number of cycles, and (2) unlike AIM that requires additional modules, such as LUTs and multiplexers, we repurpose the existing resources (i.e., memory array and peripherals) to perform the required computation, and thus, avoiding extra hardware overhead. Details are discussed in Sections \ref{subbytes} and \ref{mixColumns}.

%\vspace{-0.2cm}
%Of the 32 columns where the rest of the data are located, the plaintext matrix occupies the first four rows. The 11 key matrices occupy the next 44 rows, and the last 6 rows are used to store the intermediate data.

\begin{figure*}[htp]
\vspace{-0.0cm}
\centerline{\includegraphics[width=6.5in]{Implementation/fusedSubBytesShiftRows-v2.pdf}}
\vspace{-0.3cm}
\caption{Fusion of the \emph{SubBytes} and \emph{ShiftRows} stages for the third row of the data matrix.}
\label{fused}
\vspace{-0.5cm}
\end{figure*} 

\vspace{-0.3cm}
\subsection{AddRoundKey}
\vspace{-0.1cm}
% \jynote{Explain to ourselves: how dose the decoder stop when the other decoder is activating one word-line.}

% \esnote{Mention the Cache Automaton SA performance improvement feature, cite it, and that we use tis feature. Add it where appropriate in this section}\\
\emph{AddRoundKey} receives two matrices, the data matrix (i.e., the plaintext) and the key matrix (i.e., the round key).
Each corresponding byte in the data matrix is bit-wise $\text{XOR}$ed with each byte in the key matrix by activating two rows using two decoders.
We follow the bitline XOR functionality implementation in \cite{xieSecuringEmergingNonvolatile2018}, which costs 3 times longer than a single subarray read/write access.
%\esnote{Explaining the subarray will get a full set of SAs. Let's modify it after the evalaution is finalized} 
%The parallel column bit sensing can be achieved by precharging all the bitlines of the subarray at the same time \cite{subramaniyanCacheAutomaton2017}.

As depicted in Figure \ref{overall} (b), the data matrix (green area) and the key matrices (orange area) rows are arranged in consecutive rows (column-aligned) in the subarray, and the elements within the same row in the matrix are located next to each other horizontally in the subarray (i.e., each 128-bit data matrix or 128-bit round key requires 4 consecutive rows and 32 consecutive columns). 
This means that \emph{Sealer} can perform the bitwise $\text{XOR}$ in parallel on 192 bits (4 elements in one row of a \emph{Tile}, across 6 \emph{Tiles} in a subarray) of plaintext within one subarray in only 3 cycles (note that several subarrays can work all in parallel without almost any performance overhead!).
The \emph{AddRoundKey} output (i.e., the bitwise XOR) is sensed in the SAs (Figure \ref{overall} (c)) by activating the equivalent rows in the data matrix and key matrix. 
To maximally utilize the data retained in the sense amplifier (i.e., row buffer hit) and eliminate unnecessary write cycles, we perform the computation of the next stage on the output of the first row before writing it back to subarray.

%We find that the designed data layout combined with our proposed \emph{fused SubBytes and ShiftRows} mechanism can significantly reduce the number of operating cycles and eliminate the need for data layout reconfiguration in the middle of computation (details in Section \ref{subbytes}).

%By activating the first row in the data matrix and the first row in the key matrix simultaneously, the corresponding cells in the activated bitline will be sensed by the sense amplifier and the XOR logic, shown in Figure \ref{overall} (c), bitwise $\text{XOR}$.

%, and then, we move forward to XORing the second row of the data matrix and the key matrix. 


%Due to the high parallelism of the cache processing, we can compute a row (32 bits) in parallel within the time slot spent in one $\text{XOR}$ operation.
%After 4 time slots, each byte in the data matrix completes an $\text{XOR}$ operation with the key matrix.
%Note that for efficiency, we do not immediately write the result back to the subarray from the read buffer.
% At the beginning of the second time period, the $\text{XOR}$ result is grabbed by the next step SubBytes.

\vspace{-10pt}

\subsection{Fused SubBytes and ShiftRows} \label{subbytes}
\vspace{-0.1cm}
To efficiently\enlargethispage{5pt} implement the \emph{SubBytes} and \emph{ShiftRows} stages and reduce the total number of processing cycles, we fuse the \emph{ShiftRows} and \emph{SubBytes} stages by selecting the right order of the elements from the output of \emph{AddRoundKey} and feeding the element as the input address of the decoder to read the substitution value. The order is determined by the number of shifts required in the \emph{ShiftRows} stage.

AES defines a substitution box (S-box), which consists of a $16\times16$ byte matrix and is used to substitute each byte of the data block with the corresponding byte in the S-box matrix by using the four MSB bits to select one of the 16 rows and the four LSB bits to choose one of the 16 columns. 
Instead of adding LUTs and incurring the extra hardware overhead, \emph{Sealer} re-purposes the existing resources in SRAM and stores the S-box in the same subarray as data block and keys are stored. We accordingly reorganize the conventional $16\times16$ byte matrix to a matrix of $256\times1$ where each row represents one byte (Figure \ref{overall} - blue S-box matrix). 
We then use the result of \emph{AddRoundKey} stage, which is already stored in SAs, as the input of the decoder and read the substitution bytes consecutively.
The input of the decoder is equipped with a two 8-bit entry FIFO buffer, to enable the in-place substitution (\emph{SubBytes}) and shifting (\emph{ShiftRows}). 

%The \emph{ShiftRows} step performs the following operations on the output of the \emph{SubBytes} stage (Figure \ref{AES_flow}, Matrix D1 to D2); the first row remains unchanged, the second row is cyclic left-shifted by 1 byte, the third row is cyclic left-shifted by 2 bytes, and the fourth row is cyclic left-shifted by 3 bytes.
\begin{comment}
\begin{enumerate}
    \item First row remains unchanged.
    \item Second row: cyclic left shift by 1 byte.
    \item Third row: cyclic left shift by 2 bytes.
    \item Fourth row: cyclic left shift by 3 bytes.
\end{enumerate}
\end{comment}
%The SA can then sense the corresponding byte and store the S-box substituted data in the buffer.
Figure \ref{fused} demonstrates how the proposed \emph{fused SubBytes and ShiftRows} stage works for the third row in the data bock matrix using a step-by-step example. 
In the initial time step (T0), the XOR results of the third row in the data matrix (a1, 46, f6, 2e) and the third row of the round key matrix (cd, 4b, 42, cf) are written into the SA buffers (6c, 0d, b4, e1). 
We first explain the conventional computation in prior work (i.e., consecutive \emph{SubBytes} and \emph{ShiftRows}), and then describe the proposed fused approach in \emph{Sealer}. 

Assume that the substitution bytes (i.e., the output of the \emph{SubBytes} stage) for (6C, 0d, b4, e1) are (50, d7, 8d, f8). The output of the \emph{SubBytes} will be the input of \emph{ShiftRows} in the next stage. Because the computation is performed on the third row, the \emph{ShiftRows} stage will shift the byte to the left two times using cyclic shift, i.e., the output of the \emph{ShiftRows} stage will be (8d, f8, 50, d7).

In the proposed fused approach, we first select the element that its corresponding substitution byte will be located on the right-most side of the array after the \emph{ShiftRows} stage is completed, i.e., $sel = 10 (``0d")$ will be read into the input buffer. Then, we select the elements in the \emph{AddRoundKey} output one by one according to their corresponding locations in the \emph{ShiftRows} output from the right-most side element to the left-most side element in the array, i.e., $sel = 10 (0d) \to 11 (6c)\to 00 (e1) \to 01 (b4)$.

For the correct functionality, the input buffer should have two entries. In T1, 0d and 6c are read to the FIFO buffer. Then, the decoder takes 0d as the input address and the corresponding substitution byte is read into the row buffer (i.e., d7). In T2, first, e1 is selected (Sel = 00) and read into the second entry of the input buffer. Then, the intermediate output is shifted to the right by one byte, and finally, the decoder takes 6c as the input and the corresponding substitution byte is read into the row buffer (i.e., 50).
In T3, first, b4 is selected (Sel = 01) and read into the second entry of the input buffer. Then, the intermediate output is shifted to the right by one byte, and finally, the decoder takes e1 as the input and the corresponding substitution byte is read into the row buffer (i.e., f8).
In T4, first, the intermediate output is shifted to the right by one byte, and then, the decoder takes b4 as the input and the corresponding substitution byte is read into the row buffer (i.e., 8d). 
In T5, the intermediate buffer is shifted to the right by one byte and the final output 
% of the \emph{ShiftRows} 
is generated and ready to be used by the \emph{MixColumns} stage.% (i.e., \emph{MixColumns}). 

The shift operation is implemented by introducing a latch and a multiplexer within the SA \cite{gencache}, as shown in Figure \ref{overall}(c).
The proposed fusion approach greatly reduces write cycles, thus reducing processing latency.
% (evaluated in Section \ref{PerformanceAnalysis}).
It is important to note that the fused \emph{SubBytes} and \emph{ShiftRows} computation are done in parallel across all the \emph{Tiles} (i.e., one data block in each \emph{Tile} as the data blocks within one \emph{Tile} cannot be processed in parallel) in and across subarrays.  
%\esnote{I think the text was misleading in the last paragraph. I clarified.}
%\jynote{Very clear to understand! Just one question. You mentioned that "the fused \emph{SubBytes} and \emph{ShiftRows} computation are done in parallel across all the \emph{Tiles}". How do we achieve this in parallel? I think we have only two decoders, if we perform the SubBytes stage, one wordline will be activated to fetch according byte in S-Box. In meantime, we cannot run other Tiles, since other tiles may need different wordline to be activated. "Across subarrays" is ok, but within the same subarray, I think only one fused stage can be performed at a time.}


%Take Figure \ref{overall}(d) as an example, we need to firstly get the XORed results {6c,0d,b4,e1} through the S-box to get the substituted results \{50,d7,8d,f8\} and then arrange them into \{8d,f8,50,d7\} in the SA buffer without extra subarray accesses.
%By using the shift operation in the SA buffer, we can make the data arrive at the final location of the ShiftRows step, greatly reducing the time overhead.
%The shift operation here is implemented by introducing a latch and a multiplexer within the SA \cite{nagGenCacheLeveragingInCache2019}, as shown in Figure \ref{overall}(c).
% The Tri gate is also added into the SA logic to ensure no data will input SA when the shift operation is performing.
%When the SA performs the shift operation, the MUX will choose the input $S_{i-8}$ from the 8-th previous bitline and store it locally.


%First, we grab the bytes into the S-box in a specific order. Suppose each byte in the row need to be shifted $n$ bytes to the left, then we use the (4-n)-th element as input and take other bytes to the left. If there is no byte on the left, then the fetching will perform from the far right to the left. Take Figure \ref{overall}(d) as an example, since this row is the third row of the data matrix and needs to be shifted left by 2 bytes, we start fetching from the second element (0d). When the element passes through the S-box, the substituted result is saved in the SA buffer, located to the left of the original four data, as shown in cycle 1. Meanwhile, at cycle 1, we put the next element to be substituted by S-box into the FIFO of the decoder. At this point, we shift these 5 bytes one byte to the right, as shown in cycle 2. Then we input 6c into the S-box again and perform a right shift of one byte after getting the substituted data (50). After substituting and right-shifting all 4 data in the S-box, the final arrangement of the data in the SA buffer is the one we should get in the ShiftRows step, as shown in cycle 5. Finally, we write the last four data into the subarray to complete the ShiftRows step. Note that in cycle 2, the rightmost byte (e1) needs to be put into the decoder's FIFO during the right shift operation to ensure the completeness of the step. This explains why we need a FIFO of depth 2.


%The group length of AES is 128 bits, or 16 bytes, with the high 4 bits of each byte used as row values and the low 4 bits as column values. 
%The values of the selected rows and columns are looked up from the S-box as output.
%For the 16 bytes input of AES.
%Each one of them is mapped to a new byte as described above, called byte substitution.
%The S-box, which is an important component of the SubBytes step, can be implemented in hardware in various ways.

%Here, to further exploit the high parallelism of in-store computation and to reduce the communication overhead between subarrays, we use the free cells within the same subarray to inherently form the S-box.

%At the beginning of the SubBytes step, the data after XOR operation is put from the read buffer into the input FIFO of the decoder whose depth is 2. This FIFO ensures the feasibility of the ShiftRows step which will be introduced in Section IV.C. 
%Since we have converted the S-box from the original 16x16 matrix to a 256-row of the 8-bit matrix, the decoder can activate the corresponding word-line after receiving the 8-bit data from the input FIFO using the 8:256 multiplexer. 


% The address decoder of the subarray receives the address and translates the highest four bits of the byte into the row index and the lowest four bits into the column index
% When corresponding word lines and bitlines are activated, the pre-stored byte of S-box will be sensed by SA and the output byte will be temporarily stored in the buffer of SA.
% Note that after obtaining the substituted byte, we send the byte to two places, different from its original location in the SA. One is that, for the subsequent ShiftRows step, we put the byte output from the S-box into a shifted location of buffer in the SA after the block becomes available (bytes in the first row of the data matrix do not shift), which can then be written into the subarray to overwrite the original data. 
% In this way we achieve the fusion of the SubBytes and ShiftRows steps.
% On the other hand, the byte output from the S-box is transmitted to a small buffer, and a simple left-shift operation is performed to prepare the data for the subsequent MixColumns step.

%\subsection{ShiftRows} \label{shiftrows}


\vspace{-10pt}

\subsection{MixColumns} \label{mixColumns}
\vspace{-0.1cm}

In\enlargethispage{5pt} the \emph{MixColumns} stage, each column of the input data matrix (i.e., the output matrix of \emph{ShiftRows} stage) is multiplied with a two-dimensional constant array, called the fixed matrix, to obtain the corresponding output column.
All the addition and multiplication are both defined over a finite field. 
To achieve efficient computation in SRAM, and to reduce the resource consumption and the number of SRAM accesses for intermediate results, we decompose the matrix multiplication of data columns and the fixed matrix into matrix elements, an intermediate value $T_c$, and the product of matrix elements, following \cite{xieSecuringEmergingNonvolatile2018}.
The decomposition equation is as follows: 
\begin{equation}\label{equ:matrix}
    \scalebox{0.72}{%
\ensuremath{
\left[\begin{matrix}
2 & 3 & 1 & 1\\
1 & 2 & 3 & 1\\
1 & 1 & 2 & 3\\
3 & 1 & 1 & 2
\end{matrix}\right]
\left[\begin{matrix}
B_{0,c} \\
B_{1,c} \\
B_{2,c} \\
B_{3,c} 
\end{matrix}\right]
 =
\left[\begin{matrix}
2 B_{0,c}+3 B_{1,c}+ B_{2,c}+ B_{3,c} \\
B_{0,c}+2 B_{1,c}+3 B_{2,c}+ B_{3,c} \\
B_{0,c}+B_{1,c}+2 B_{2,c}+3 B_{3,c} \\
3 B_{0,c}+B_{1,c}+ B_{2,c}+2 B_{3,c} 
\end{matrix}\right]
\\
= 
\left[\begin{matrix}
T_c \oplus 2 B_{0,c} \oplus 2 B_{1,c} \oplus B_{0,c} \\
T_c \oplus 2 B_{1,c} \oplus 2 B_{2,c} \oplus B_{1,c} \\
T_c \oplus 2 B_{2,c} \oplus 2 B_{3,c} \oplus B_{2,c} \\
T_c \oplus 2 B_{0,c} \oplus 2 B_{3,c} \oplus B_{3,c}, 
\end{matrix}\right]}%$%      
        }
\end{equation}
% \esnote{scale down the size of these matrices.}\jynote{done.}
where $B_{r,c}$ denotes the byte in row $r$ and column $c$, and $T_c$ is the intermediate result for column $c$. $T_c$ is calculated as: 
\begin{equation}
%\vspce{-0.2cm}
    T_c=B_{0,c}\oplus B_{1,c} \oplus B_{2,c} \oplus B_{3,c}.
\end{equation}
% Multiplication by 3 can be replaced with a multiplication with two and an XOR operation \cite{xieSecuringEmergingNonvolatile2018}. Therefore, we can decompose the matrix multiplication as follows:
% \begin{equation}
%     B^{'}_{r,c}=T_c \oplus 2  B_{(r+1)mod(4),c} \oplus 2  B_{r,c} \oplus B_{r,c}\\ 
% \end{equation}
% where $B$ denotes the byte in row r, column c and $T_c$ is the intermediate result for each column. 

The computation of $2\times B_{r,c}$ elements in Equation \ref{equ:matrix} is done in \emph{ShiftRows} stage by shifting the output of \emph{ShiftRows} stage to the left by one bit and storing them back in the intermediate region of the subarray. 
Figure \ref{mixcolumn}(a) shows how $T_c$ in each column is calculated and stored in the subarray in 6 steps using an example (note that the calculation of $T_c$ is fully parallel in each column). % of XOR and write operations.
%, similar to \cite{xieSecuringEmergingNonvolatile2018},
To calculate $T_0$, in Step 1, the two (red) worldlines are activated simultaneously to calculate the XOR of $B_{0,0}$ and $B_{1,0}$, and store the result ($I_0$) in the intermediate region in Step 2. Next, the XOR of $B_{2,0}$ and $B_{3,0}$ is calculated in Step 3 and written back to the array ($I_1$) in Step 4. Finally, $T_0$ is calculated (Step 5) and written back (Step 6). % in Step 5 and 6, respectively. 
Figure \ref{mixcolumn}(b) shows how the final output is calculated for $T_c \oplus 2 B_{0,c} \oplus 2 B_{1,c} \oplus B_{0,c}$ by activating the corresponding rows, calculating the XOR of the activated cells, and writing the intermediate results back. After 6 steps, the output of the \emph{MixColumn} ($B^{'}_{0,0}$) overwrites input ($B_{0,0}$).
%To obtain the final output matrix in the MixColunms stage, the XOR among the corresponding $T_c$, the products of matrix B elements and 2, and each byte itself, as in Equation \ref{equ: matrix}. 
%As shown in Figure \ref{mixcolumn}(b), again after 6 steps of XOR and WRITE operations, the output bytes ($B^{'}_{0,0}$) of the MixColumn will be written to its original position in the subarray, overwriting the original data ($B_{0,0}$).

\vspace{-0.15cm}
\section{Key generation and Storage}
\vspace{-0.1cm}
%\esnote{We need to explain how master key (initial key) and round keys are generated and stored.}
%\jynote{I have added an implementation of key generation using in-cache computing, which has been briefly introduced here.}
Similar to state-of-the-art memory encryption engines~\cite{gueronMemoryEncryptionEngine2016b}, we assume the encryption key is generated using a hardware random number generator and implemented in the processor chip. The key is inaccessible outside of the chip.
% The hardware random number generator in the processor chip \cite{gueronMemoryEncryptionEngine2016}, or t
The expansion of the given cipher key can also be utilized to obtain 11 partial keys, which are used in the initial round, the 9 main rounds, and the final round.
The expansion process can be implemented in the subarray, including shift operations between columns, the \emph{SubBytes} stage, the XOR operations between rows and a given reconstruction matrix.
%These steps and operations have been discussed above, which is easy to be applied here to generate keys.
The generated keys will be stored within the subarray (Figure \ref{overall}).

%\section{System Integration}

%Re-purposing L3 cache 
%How to avoid interfering with the normal cache operation 
%What changes are necessary in the cache controller and SW 
%Cache controller, ISA, how many parallel subarrays, prefetching, and encryption on prefetched data 

%\vspce{-0.1cm}

==> islped22-1/Introduction/intro.tex <==
% \vspace{-0.2cm}
\section{Introduction}
\vspace{-0.1cm}
% Intel SGX. The processor is trusted, but the bus and memory is not. 

% ORAM tries to address confidentiality, but it is expensive (address encryption is a future work) 

%To improve the performance, other in-memory solutions are proposed (such as AIM). However, they perform bulk encryption in NVRAM, but bus is still untrusted 

% Also briefly mention InvisMem. This expand the trusted region to the logic layer of the memory and our approach does not 

%To address the performance issue and the untrusted bus/memory issue, we presented Sealer, an in-SRAM encryption engine, which utilizes intrinsic parallelism of cache subarrays for fast and efficient encryption and decryption

%Need for fast encryption engine 
Healthcare organizations, businesses, and governments rely heavily on secure computer systems for their daily activities and business conduct.
To provide data confidentiality, a wide range of computational devices, from high-end servers to low-power IoT devices, implement data encryption standards. 
%Security and privacy protection are an essential part of computer systems. 
%Security and privacy protection is not just for software, but trusted hardware is critical. 
%In order to make the information transmitted in the hardware trustworthy and to prevent attackers from gaining access to confidential information by eavesdropping on the circuit, data is only transmitted in the circuit or stored in the storage module after it has been encrypted. 
In these devices, only the processor chip is considered secure and trusted hardware in the system \cite{costanIntelSgxExplained2016}. Anything outside the processor chip boundary is typically assumed vulnerable and untrusted. In such a threat model, any data sent off-chip (i.e., to the memory or on the cloud) is potentially at risk of being manipulated, tampered with, or leaked~\cite{haldermanLestWeRemember2009b}. Novel memory technologies, such as Non-Volatile Memories (NVMs), can retain data for a long time after power loss, thus, making memory protection even more critical. 
%In addition, memory bus (which connects processor chip to the main memory) can be easily probed by an adversary to extract data or access pattern~\cite{gueronMemoryEncryptionEngine2016b}.

To protect against memory and bus attacks (e.g., bus snooping and cold boot attacks \cite{haldermanLestWeRemember2009b}), processor vendors are increasingly adding support for protecting the integrity and confidentiality of data through integrity verification and encryption on the on-chip memory controller \cite{gueronMemoryEncryptionEngine2016b,kaplanAMDMemoryEncryption2016a}.
%\cite{hensonMemoryEncryptionSurvey2014b}
%\cite{haldermanLestWeRemember2009b}
%(e.g., before data leaves the chip)
%~\cite{gueronMemoryEncryptionEngine2016b,kaplanAMDMemoryEncryption2016a}.
Memory encryption typically uses Advanced Encryption Standard (AES) block cipher to encrypt plaintext going to or decrypt ciphertext from the main memory, using a key re-generated on each system reboot. However, real-time encryption or decryption at every memory access in the critical path results in severe performance overhead \cite{mathew53GbpsNativeGF2010}. 
%\esnote{maybe adding more and stronger motivation of why faster encryption}\hnnote{I think the fact that it is on critical path should be sufficient. I could not find any paper that shows this with numbers or even references. If I find, I'll add it here.}.

To address the performance issue, recent prior works have proposed in-memory and near-memory encryption/decryption solutions~\cite{xieSecuringEmergingNonvolatile2018,agaInvisiMemSmartMemory2017,angiziPIMALogicNovelProcessinginmemory2018}. %,angiziRIMPANewReconfigurable2017}. 
% \cite{xieSecuringEmergingNonvolatile2018,agaInvisiMemSmartMemory2017,angiziPIMAlogicNovelProcessinginmemory2018,angiziRIMPANewReconfigurable2017}.
Xie et al.~\cite{xieSecuringEmergingNonvolatile2018} propose AIM, an in-memory AES engine that provides bulk encryption of data blocks in NVM for mobile devices, and encryption is executed only when the device is shut down or put into sleep/screen-lock mode. Despite its computational efficiency, AIM does not protect data confidentiality against bus and memory attacks. Aga et al.~\cite{agaInvisiMemSmartMemory2017} present InvisiMem, which uses the logic layer in 3D stacked memory to implement cryptographic primitives.
%for data confidentiality. 
However, the InvisiMem design expands the trusted computing base (TCB) to the logic layer of the memory. To protect data confidentiality against physical attacks on both memory and bus, an efficient real-time encryption/decryption engine needs to be implemented on the processor chip.% (to avoid expanding the TCB).


To provide a low-cost, and real-time on-chip encryption engine, for the first time, this paper proposes to re-purpose 6T SRAM subarrays into active large vector computational units to perform encryption and decryption on-chip. Our solution, \textit{Sealer}, exploits intrinsic parallelism and bitline computational capability of memory subarrays for fast and low-overhead AES implementation, and incurs only a negligible area overhead (less than 1.55\%) compared to the traditional SRAM arrays. 
%present Sealer, an in-SRAM AES encryption engine which utilizes intrinsic parallelism of cache subarrays for fast and efficient encryption and decryption. Using massive parallelism and emerging bitline SRAM technology, it is possible to re-purpose existing cache elements (with little or no extensions to the existing cache structures) into active large vector computational units to perform encryption and decryption on the chip. By encrypting and decrypting data in the cache (on the chip), Sealer does not expand the TCB of system. 
%\textit{Sealer} provides data confidentiality against both bus and memory attacks by real-time memory encryption on the chip for every cache line sending off-chip and can be adopted for data/code encryption on a wide variety of computational devices, ranging from embedded devices to high-end servers. 
% Moreover, 
\textit{Sealer} provides the same level of memory confidentiality as Intel Memory Encryption Engine (MEE)~\cite{gueronMemoryEncryptionEngine2016b} or AMD Secure Memory Encryption (SME)~\cite{kaplanAMDMemoryEncryption2016a}, and unlike InvisiMem, does not extend the TCB.
\textit{Sealer} can act as conventional SRAM when the encryption/decryption is unnecessary.
%but yields higher performance and energy efficiency.
%Moreover, unlike InvisiMem, Sealer does not extend the TCB.

In summary, the paper makes the following \textbf{contributions:}
\begin{itemize}
    \item We present \textit{Sealer}, a real-time in-SRAM AES engine to provide data confidentiality by encrypting the plaintext on the CPU chip.
    %and narrowing the TCB. 
    Our proposed architecture effectively stores the required data 
    %and matrices 
    for encryption into the same 
    %SRAM
    subarray. This allows the peripherals and resources to be shared among different computation and communication units, thus, reducing performance and hardware overhead. 
    %and prevent physical attacks, such as bus snooping and cold boot attacks. Our design requires minimal change to the SRAM array structure.   
    %\item ... by narrowing the trusted computing base (TCB) to the inside of the CPU package ... to ensure confidentiality ... encrypts the plaintext using AES algorithm and sends the encrypted data to DRAM.
    \item We present an algorithm and architecture methodology to efficiently map the AES algorithm to the \emph{Sealer} architecture. By fusing the \textit{SubBytes} and \textit{ShiftRows} stages in AES, we can interleave the computation at a finer granularity and maximally exploit on-the-fly computation to significantly reduce data movement and \textit{write} cycles.
    %and the number of write cycles into the subarrays.  
    \item We compare \textit{Sealer} with several on-chip and in-memory AES encryption engines and show that our solution has up to 323$\times$ performance improvement, up to 91$\times$ throughput-per-area improvement, and 3$\times$ lower energy consumption compared to prior solutions. To separate the architectural and technology contribution of \textit{Sealer}, we evaluate an in-NVM AES engine on SRAM (\emph{AIM-SRAM}) and find that our solution achieves 6$\times$ higher performance than AIM-SRAM due to architectural contribution and 18$\times$ better performance due to technology benefits.
\end{itemize}

%\jynote{
%\begin{itemize}
    %\item Improving the performance and enhancing confidentiality of existing bulk encryption by carefully transferring the encryption mechanism from memory to SRAM considering the inherent characteristics of SRAM.
    %\item The conventional encryption mechanism is adapted on SRAM and the algorithm process is improved. Specifically, SubBytes and ShiftRows stages in AES are fused, allowing the two stages to interleave at a finer granularity, significantly reducing data movement.
   % \item With minimal hardware overhead, conventional SA has been extended with the ability to perform basic logic operations ($and$, $nor$, $xor$) and shift operations.
    %\item We compare the proposed architecture in detail with existing architectures in terms of performance, throughput, and energy consumption. We also construct a variant of the existing scheme in SRAM to further compare the performance improvements resulting from the architecture change.
%\end{itemize}
%}

\begin{comment}

can be adopted for data/code encryption on a wide variety of computational devices, ranging from embedded devices to high-end servers. 

    \item Minimal changes to the cache structure. We reuse the SRAM arrays for LUT operations required for AES  instead of adding LUT logics.
    \item Fusion of \emph{SubBytes} and \emph{ShiftRows} steps in AES. Before writing back intermediate results, we perform SubBytes and \emph{ShiftRows} steps together and then write final results into subarray, which significantly reduces the data movement.
  %  \item Overall area overhead is trivial. The implementations of LUT and shift operations induce only 2 more gates in each sense amplifier (SA).

 \item Sealer guarantees data confidentiality to prevent physical attacks (e.g. bus snooping, cold boot, …). \emph{Sealer} provides real-time memory encryption for every cache line/memory access and for every computing platform including PC and servers (rather than bulk encryption in mobile phones (AIM paper) only when the phone is locked). \emph{Sealer} is scalable from embedded to high-end servers.
 %\item  Sealer provides the baseline MEE equivalent guarantee for memory confidentiality, but with higher performance and energy efficiency (using in-cache computing). We can mention that we can have the same level of protection as Intel MEE  or AMD SME, but we need to evaluate our performance with those designs just for confidentiality part (there is no performance evaluation in Intel and AMD whitepapers). One additional note: Intel also has TME which encrypts the whole memory of the system.





% In order to achieve trusted computing, Intel has proposed a new technology Software Guard Extensions (SGX) since 2015 to run software in a secure and trusted way inside a closed computer system \cite{gueronMemoryEncryptionEngine2016}. 
% This technology can be found implemented in Intel's Skylake processors.
% SGX enables a trusted CPU by narrowing the security perimeter to the inside of the CPU package and using the concept of an "enclave" which is similar to the "container" concept to prevent applications running inside from being accessed by higher privileges, including the OS kernel \cite{anatiInnovativeTechnologyCPU,mckeenInnovativeInstructionsSoftware2013}. 
% The codes with SGX are run in separate enclaves, and to enable the secret owner to provide secrets to the enclave, SGX provides a trusted channel between the untrusted memory and the trusted CPU. 
% The Memory Encryption Engine (MEE) which is located in the CPU side is responsible for ensuring the confidentiality, integrity and freshness of the data in this channel. 
% The MEE uses the Advanced Encryption Standard (AES) algorithm to encrypt the plaintext to guarantee confidentiality.
% The encrypted data is sent to DRAM in a certain structure to ensure integrity and freshness. 
% However, due to the area of the CPU and the power consumption shows that the hardware used by the MEE to perform the AES algorithm to achieve encryption is not very efficient.

In order to achieve trusted computing, Intel proposed the Software Guard Extensions (SGX) technology to implement a trusted hardware \cite{gueronMemoryEncryptionEngine2016}. 
By narrowing the trusted computing base (TCB) to the inside of the CPU package, SGX provides high-level security with the concept of "enclave". 
For data communication between CPU and DRAM, SGX uses Memory Encryption Engine (MEE) to ensure confidentiality, integrity, and freshness of the data, which encrypts the plaintext using AES algorithm and sends the encrypted data to DRAM.
However, due to the limitation of CPU area and power, the dedicated hardware used by MEE is not so efficient.


In order to improve the efficiency of encryption, some methods using in-memory computing have been proposed \cite{xieSecuringEmergingNonvolatile2018,agaInvisiMemSmartMemory2017,angiziPIMAlogicNovelProcessinginmemory2018,rimpa}. AIM in \cite{xieSecuringEmergingNonvolatile2018} proposes a high-speed and efficient in-memory implementation of AES to address the vulnerability problem encountered by NVMM. 
AIM transfers the AES encryption execution process from the low-paralleled CPU to the high-paralleled nonvolatile main memory (NVMM). 
AIM uses three different parallelism levels: chip-level, bank-level, and subarray-level to obtain different degrees of acceleration. 
By efficiently mapping AES algorithms inside nonvolatile memory (NVM) with extra peripheral circuits, AIM can fully utilize the parallelism capability provided by NVM, significantly reduce the data movement, satisfy the high bandwidth requirement of AES to achieve the efficient implementation of AES algorithms.
What's more, PIMA-Logic \cite{angiziPIMAlogicNovelProcessinginmemory2018} proposes an in-memory computing architecture based on Spin-Orbit Torque Magnetic Random Access Memory (SOT-MRAM) for highly flexible and efficient logic computation. 
PIMA-Logic implements Boolean logic function computation between different rows and columns with low hardware overhead, which significantly reduces data movement. 
The simulation results show that PIMA-Logic outperforms CMOS-ASIC and other implementations.
However, the above approaches do not encrypt the data between CPU-DRAM. 
Once an attacker can manage to eavesdrop on the CPU-DRAM buses, there is no way to keep the data confidential, which means the system cannot be trusted.
InvisiMem \cite{agaInvisiMemSmartMemory2017} leverages the computational characteristics of 3D stacked memory to secure address and data confidentiality, data integrity, and freshness for computing systems. However, InvisiMem extends the TCB to include the logic layer of memories, increasing the attack surface, and the overall security performance of InvisiMem remains to be evaluated in long term.

% To improve the encryption efficiency, some methods to perform the computation inside the memory module have been proposed. Among them, AIM proposes a high-speed and efficient in-store implementation of AES for the vulnerability problem encountered by NVMM. By exploiting the characteristics of NVM itself, this method can encrypt data stored in NVM efficiently. However, this method does not encrypt the data communication between CPU-DRAM. Once an attacker can manage to eavesdrop on the CPU and DRAM buses, there is no way to keep the data confidential.

Thus, to address the performance issue and the untrusted bus/memory issue, we presented \emph{Sealer}, an in-SRAM encryption engine, which utilizes intrinsic parallelism of cache subarrays for fast and efficient encryption and decryption. 


\end{comment}

% \vspace{-0.1cm}

==> islped22-1/Relatedwork/relatedwork.tex <==
\vspace{-0.2cm}
\section{Related Work}
\vspace{-0.1cm}
%\esnote{Some portions of the related work is not really related to our work, such as in-DRAM computation. So I commented those part. Also, I moved the "Compute Cache" portion to the background so you can clean/complete it based on the comment that I made in that section. In the related work, we want to only discuss the works that have accelerated encryption engine either with in-memory/near-memory architectures, or by adding hardware to the memory controller, or by designing an ASIC}

%\esnote{Here is what I would suggest for the background: \\ Start from the existing encryption solution, such as Intel's MME and AMD's SME, and explain them in one paragraph. Then, in the next paragraph, explain existing in-memory solutions for encryption (AIM, InvisiMem, PIMA-Logic and also briefly EE1 and EE2 that you use in the evaluation (for this, you can see the related work in the AIM paper). Also, it is not enough to only mention the related work. We need to make connection between related work and our work, and briefly discuss pros and cons, etc.}
%\jynote{Finished.}\hnnote{Jingyao, Can you please write about EE1, EE2 and DW-ES (at least one paragraph for each)? Then I will edit this related work section.} \jynote{Sure! They have been added in this section.}


%  AIM, InvisiMEM, PIMA-Logic

%To protect data confidentiality against attacks on bus or memory, processor chips are enhanced by on-chip encryption/decryption engines.

%. Several works have proposed high performance or energy efficient on-chip AES encryption engines for memory protection. 
Hämäläinen et al.\cite{hamalainenDesignImplementationLowarea2006} (EE-1) and Mathew et al.\cite{mathew53GbpsNativeGF2010} (EE-2) propose on-die AES encryption engines.
%AES encryption hardware core (EE-1).
%In their design, the AES round key expansion operations can be performed simultaneously with 8-bit data path.
%EE-1 can achieve the throughput of 232 Mbps with 3.9K gates and 62 $\mu$W/MHz.Since EE-1 is for low-cost and low-power devices, the performance is not enough for real-time encryption.
%Mathew et al.\cite{mathew53GbpsNativeGF2010} 
%fabricate the on-die AES encryption/decryption hardware core in 45nm CMOS (EE-2). They 
%design an on-die encryption engine (EE-2) and 
EE-2 computes the entire AES round in composite-field arithmetic, resulting in delay reduction in the critical S-box unit. They also use folded datapath design to reduce the wiring complexity of \emph{ShiftRows} permutations. %In addition, the fused MixColumn design uses a different matrix to reduce the overall AES round area. %However, the power consumption is up to 125 mW, decreasing the energy efficiency of the chip.
%The conventional AES design will map GF(2$^8$) to GF(2$^2$)$^2$ for S-Box computation, which limits the performance of the AES. Unlike the conventional LUT-based designs of AES, \cite{mathew53GbpsNativeGF2010} maps all the operations of the AES round in GF(2$^2$)$^2$, which remove the mapping overhead. 
Wang et al. propose DW-AES\cite{wangDWAESDomainwallNanowirebased2016} by utilizing the domain wall nanowire to implement the AES encryption algorithm in NVM. 
%The basic logical operations, such as XOR, AND, and LUT are implemented with the domain wall nanowire. 
% Though the throughput of DW-AES is 3.6x than the CMOS ASIC proposed in \cite{mathew340MV2892015}, the latency for one data block is still not low enough to make it efficient for real-time encryption. 
Though the throughput of DW-AES is 3.6$\times$ higher than the CMOS ASIC proposed in \cite{mathew340MV2892015}, the latency for one data block is still not low enough to accommodate real-time encryption. 

To improve the performance of memory encryption, recent works propose in-memory encryption architectures. Xie et al.\cite{xieSecuringEmergingNonvolatile2018} present AIM, an efficient in-NVM implementation of AES. AIM provides bulk encryption/decryption for mobile devices to protect memory content only when the device is shut down, locked, or in sleep mode. 
%AIM transfers the AES encryption execution process from the low-paralleled CPU to the high-paralleled non-volatile main memory.
%and uses three different parallelism levels: chip-level, bank-level, and subarray-level to obtain different degrees of acceleration. 
%By efficiently mapping AES algorithms inside NVM with extra peripheral circuits, AIM can fully utilize the parallelism capability provided by NVM, significantly reducing the data movement. %and satisfying the high bandwidth requirement of AES to achieve the efficient implementation of AES. 
Therefore, AIM does not provide real-time memory encryption to protect against bus and memory attacks.
Aga et al. propose InvisiMem \cite{agaInvisiMemSmartMemory2017}, which expands the trust base to the logic layer of 3D stacked memory to implement encryption. InvisiMem guarantees confidentiality, integrity, and protecting access patterns using a packetized interface and authentication to establish a secure communication channel between processor and memory. \emph{Sealer} does not expand the TCB of the system and is the first work that proposes in-SRAM encryption for data confidentiality. 
%\hnnote{I added this paragraph here and removed it from evaluation then.}\esnote{Looks good. Thanks.}


Commercial examples of memory protection solutions are Memory Encryption Engine (MEE)~\cite{gueronMemoryEncryptionEngine2016b} in Intel SGX \cite{costanIntelSgxExplained2016} and AMD's Secure Memory Engine (SME)~\cite{kaplanAMDMemoryEncryption2016a}. 
%Intel SGX is a technology that protects sensitive data and code in a secure and protected/encrypted region called "enclave".
The hardware component of SGX (i.e., MEE) protects the confidentiality, integrity, and freshness of processor-DRAM traffic for secure enclaves. The confidentiality protection in MME and SME are implemented by AES-128 encryption. %Similarly, AMD's SME provides memory encryption using AES-128 encryption engines that are implemented in on-chip memory controller.
\emph{Sealer} provides the MEE- and SME-equivalent guarantee for memory confidentiality, but with higher performance and lower area overhead by exploiting intrinsic parallelism and bitline computational capability of SRAM subarrays.

We compare the performance of \emph{Sealer} with EE-1  ~\cite{hamalainenDesignImplementationLowarea2006}, EE-2~\cite{mathew53GbpsNativeGF2010}, DW-AES~\cite{wangDWAESDomainwallNanowirebased2016}, and AIM \cite{xieSecuringEmergingNonvolatile2018} in Section~\ref{sec:evaluation}.  
We are not able to compare the performance of \emph{Sealer} with Intel's MEE, AMD's SME, and Invisimem mainly because these designs provide other memory protections, such as data integrity. Therefore, we cannot isolate the encryption performance from other components in their designs. 
%\hnnote{I think PIMA-Logic is not relevant to memory protection or encryption since all other works here are related, this is the only one that does not anything with encryption. So I remove it for now. Let me know if you think it should be there.} \esnote{I agree.}
%PIMA-Logic \cite{angiziPIMAlogicNovelProcessinginmemory2018} proposes an in-memory computing architecture based on Spin-Orbit Torque Magnetic Random Access Memory (SOT-MRAM) for highly flexible and efficient logic computation. 
%However, the above approaches do not encrypt the data between CPU-DRAM. Once an attacker can manage to eavesdrop on the CPU-DRAM buses, there is no way to keep the data confidential, which means the system cannot be trusted.

%\hnnote{Elaheh, Should we mention it here or in the evaluation section. We should also say the same thing for MEE and SME. For MEE and SME we can say that there is no performance evaluation for just encryption part. Invisimem has some performance evaluations against unsecure memory. I added a paragraph in evaluation section.}
%\esnote{Thanks, Hoda. I think it is fine to add the reason for why we are not comparing against InvisiMem here in the related work}












\begin{comment}
To protect user's confidential data, general encryption methods utilize dedicated hardware, located inside the processor chip \cite{gueronMemoryEncryptionEngine2016b} or in the main memory \cite{kaplanAMDMemoryEncryption2016a}, to accelerate encryption algorithms.
Intel has released the Software Guard Extensions (SGX) technology since 2015 to run software in a secure and trusted way inside a closed computer system \cite{gueronMemoryEncryptionEngine2016b}.
The Memory Encryption Engine (MEE), which is located on the CPU chip, is responsible for ensuring the confidentiality, integrity and freshness of the data. 
The MEE uses the AES algorithm to encrypt the plaintext to guarantee confidentiality.
The encrypted data is sent to DRAM in a certain structure to ensure integrity and freshness. 

However, due to the area of the CPU and the power consumption shows that the hardware used by the MEE to perform the AES algorithm suffers from the performance problem, as the same as \cite{hamalainenDesignImplementationLowarea2006}.
In addition to the performance problem, the dedicated hardware encryption engine also encounters the power problem \cite{mathew53GbpsNativeGF2010}.



To  improve  the  performance and efficiency,  bulk encryption/decryption has been proposed \cite{colpProtectingDataSmartphones2015,xieSecuringEmergingNonvolatile2018} to encrypt memory on edge devices.
AIM \cite{xieSecuringEmergingNonvolatile2018} presents a high-speed and efficient in-memory implementation of AES to address the vulnerability problem encountered by nonvolatile main memory (NVMM). 
AIM transfers the AES encryption execution process from the low-paralleled CPU to the high-paralleled NVMM. 
AIM uses three different parallelism levels: chip-level, bank-level, and subarray-level to obtain different degrees of acceleration. 
By efficiently mapping AES algorithms inside nonvolatile memory (NVM) with extra peripheral circuits, AIM can fully utilize the parallelism capability provided by NVM, significantly reducing the data movement and satisfying the high bandwidth requirement of AES to achieve the efficient implementation of AES.


PIMA-Logic \cite{angiziPIMAlogicNovelProcessinginmemory2018} proposes an in-memory computing architecture based on Spin-Orbit Torque Magnetic Random Access Memory (SOT-MRAM) for highly flexible and efficient logic computation. 
However, the above approaches do not encrypt the data between CPU-DRAM. 
Once an attacker can manage to eavesdrop on the CPU-DRAM buses, there is no way to keep the data confidential, which means the system cannot be trusted.


InvisiMem \cite{agaInvisiMemSmartMemory2017} address the snooping problem on the memory bus by expanding the trust base to include the chip, the memory bus, and the logic layer of 3D stacked memory, which still leave the threat unsolved.

\end{comment}
% In order to achieve trusted computing, Intel has proposed a new technology Software Guard Extensions (SGX) since 2015 to run software in a secure and trusted way inside a closed computer system \cite{gueronMemoryEncryptionEngine2016b}. 
% This technology can be found implemented in Intel's Skylake processors.
% SGX enables a trusted CPU by narrowing the security perimeter to the inside of the CPU package and using the concept of an "enclave" which is similar to the "container" concept to prevent applications running inside from being accessed by higher privileges, including the OS kernel \cite{anatiInnovativeTechnologyCPU,mckeenInnovativeInstructionsSoftware2013}. 
% The codes with SGX are run in separate enclaves, and to enable the secret owner to provide secrets to the enclave, SGX provides a trusted channel between the untrusted memory and the trusted CPU. 
% The Memory Encryption Engine (MEE) which is located in the CPU side is responsible for ensuring the confidentiality, integrity and freshness of the data in this channel. 
% The MEE uses the Advanced Encryption Standard (AES) algorithm to encrypt the plaintext to guarantee confidentiality.
% The encrypted data is sent to DRAM in a certain structure to ensure integrity and freshness. 
% However, due to the area of the CPU and the power consumption shows that the hardware used by the MEE to perform the AES algorithm to achieve encryption is not very efficient.

%Unlike near-memory computing, in-memory computing uses not only peripheral circuits close to the memory but also the memory cells and the memory array itself, further reducing data movement within the memory and increasing computation parallelism.

%By activating three wordlines in DRAM at the same time and modifying the sense amplifier (SA), Ambit enables the bulk bitwise operation to be fully implemented inside DRAM \cite{seshadriAmbitInmemoryAccelerator2017,seshadriFastBulkBitwise2015}.
%ComputeDRAM even implements AND and OR operations with unmodified DRAMs by activating multiple wordlines in rapid succession and issuing sequences of commands that violate the nominal timing specification \cite{gaoComputeDRAMInMemoryCompute2019}.
%Pinatubo implements multiple logical operations, AND, OR, XOR, INV, by making small modifications to the SA of the NVM \cite{liPinatuboProcessinginmemoryArchitecture2016}.


%One application scenario of in-cache computing is to accelerate the encryption process, taking advantage of the high parallelism and high bandwidth of in-cache computing \cite{xieSecuringEmergingNonvolatile2018,agaInvisiMemSmartMemory2017,angiziPIMAlogicNovelProcessinginmemory2018,angiziRIMPANewReconfigurable2017}.

% In order to improve the efficiency of encryption, some methods using in-memory computing have been proposed \cite{xieSecuringEmergingNonvolatile2018,agaInvisiMemSmartMemory2017,angiziPIMAlogicNovelProcessinginmemory2018,angiziRIMPANewReconfigurable2017}. 



% AIM \cite{xieSecuringEmergingNonvolatile2018} proposes a high-speed and efficient in-memory implementation of AES to address the vulnerability problem encountered by NVMM. 
% AIM transfers the AES encryption execution process from the low-paralleled CPU to the high-paralleled nonvolatile main memory (NVMM). 
% AIM uses three different parallelism levels: chip-level, bank-level, and subarray-level to obtain different degrees of acceleration. 
% By efficiently mapping AES algorithms inside nonvolatile memory (NVM) with extra peripheral circuits, AIM can fully utilize the parallelism capability provided by NVM, significantly reduce the data movement, satisfy the high bandwidth requirement of AES to achieve the efficient implementation of AES algorithms.
% PIMA-Logic \cite{angiziPIMAlogicNovelProcessinginmemory2018} proposes an in-memory computing architecture based on Spin-Orbit Torque Magnetic Random Access Memory (SOT-MRAM) for highly flexible and efficient logic computation. 
% PIMA-Logic implements Boolean logic function computation between different rows and columns with low hardware overhead, which significantly reduces data movement. 
% The simulation results show that PIMA-Logic outperforms CMOS-ASIC and other implementations.
% However, the above approaches do not encrypt the data between CPU-DRAM. 
% Once an attacker can manage to eavesdrop on the CPU-DRAM buses, there is no way to keep the data confidential, which means the system cannot be trusted.

%\vspace{-0.2cm}
